Visual Crowd Analysis: Open Research Problems

Over the last decade, there has been a remarkable surge in interest in automated crowd monitoring within the computer vision community. Modern deep-learning approaches have made it possible to develop fully-automated vision-based crowd-monitoring applications. However, despite the magnitude of the issue at hand, the significant technological advancements, and the consistent interest of the research community, there are still numerous challenges that need to be overcome. In this article, we delve into six major areas of visual crowd analysis, emphasizing the key developments in each of these areas. We outline the crucial unresolved issues that must be tackled in future works, in order to ensure that the field of automated crowd monitoring continues to progress and thrive. Several surveys related to this topic have been conducted in the past. Nonetheless, this article thoroughly examines and presents a more intuitive categorization of works, while also depicting the latest breakthroughs within the field, incorporating more recent studies carried out within the last few years in a concise manner. By carefully choosing prominent works with significant contributions in terms of novelty or performance gains, this paper presents a more comprehensive exposition of advancements in the current state-of-the-art.

==> biographies/hamid.tex <==

% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{hamid.jpg}}]{Hamid Menouar} (SM’16) is a Senior Research and Development Expert at Qatar Mobility Innovations Center (QMIC), Qatar, where he leads the development of innovations in the area of smart cities and smart living.  
% Before moving to Qatar in 2010, Hamid worked for 8 years at Hitachi research lab in Sophia Antipolice, France, where he contributed and led research and development activities related to connected vehicles. During his experience with Hitachi, he has heavily contributed to the development of connected vehicles communication standards in Europe through an active participation at ETSI TC ITS and Car to Car Communication Consortium.  
% Hamid received the Engineering degree (M.S.) in computer science from the University of Science and Technology Houari Boumediene, Algiers, Algeria, in 2003, the DEA (M.S.) degree in systems and information technologies from the University of Technology of Compiegne, France, 2004, and the Ph.D. degree in computer science from Telecom ParisTech, Paris, France, in 2008. 
% \end{IEEEbiography}

% \begin{wrapfigure}{l}{23mm} \includegraphics[width=1in,height=2.2in,clip,keepaspectratio]{biographies/hamid.jpg} \end{wrapfigure}
\textbf{Hamid Menouar} (SM’16) is a Senior Research and Development Expert at Qatar Mobility Innovations Center (QMIC), Qatar, where he leads the development of innovations in the area of smart cities and smart living. Before moving to Qatar in 2010, Hamid worked for 8 years at Hitachi research lab in Sophia Antipolice, France, where he contributed and led research and development activities related to connected vehicles. During his experience with Hitachi, he has heavily contributed to the development of connected vehicles communication standards in Europe through an active participation at ETSI TC ITS and Car to Car Communication Consortium. Hamid received the Engineering degree (M.S.) in computer science from the University of Science and Technology Houari Boumediene, Algiers, Algeria, in 2003, the DEA (M.S.) degree in systems and information technologies from the University of Technology of Compiegne, France, 2004, and the Ph.D. degree in computer science from Telecom ParisTech, Paris, France, in 2008. 


==> biographies/hamila.tex <==
% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{hamila.jpg}}]{Prof. Ridha Hamila} received the MSc, LicTech with distinction, and PhD degrees from Tampere University of Technology (TUT), Tampere, Finland, in 1996, 1999, and 2002, respectively. Dr. Hamila currently a Full Professor at the Department of Electrical Engineering, Qatar University, Qatar. From 1994 to 2002 he held various research and teaching positions at TUT within the Department of Information Technology, Finland. From 2002 to 2003 he was a System Specialist at Nokia research Center and Nokia Networks, Helsinki. From 2004 to 2009 he was with Emirates Telecommunications Corporation, UAE. Also, from 2004 to 2013 he was adjunct Professor at the Department of Communications Engineering, TUT. His current research interests include mobile and broadband wireless communication systems, Mobile Edge Computing, Internet of Everything, and Machine Learning. In these areas, he has published over 200 journal and conference papers most of them in the peered reviewed IEEE publications, filed seven US patents, and wrote numerous confidential industrial research reports.  Dr. Hamila has been involved in several past and current industrial projects, Ooreedo, Qatar National Research Fund, Finnish Academy projects, EU research and education programs. He supervised a large number of under/graduate students and postdoctoral fellows. He organized many international workshops and conferences. He is a Senior Member of IEEE.
% \end{IEEEbiography}


% \begin{wrapfigure}{l}{23mm} \includegraphics[width=1in,height=2.4in,clip,keepaspectratio]{biographies/hamila.jpg} \end{wrapfigure}
\textbf{Ridha Hamila} received the MSc, LicTech with distinction, and PhD degrees from Tampere University of Technology (TUT), Tampere, Finland, in 1996, 1999, and 2002, respectively. Dr. Hamila is currently a Full Professor at the Department of Electrical Engineering, Qatar University, Qatar. From 1994 to 2002 he held various research and teaching positions at TUT within the Department of Information Technology, Finland. From 2002 to 2003 he was a System Specialist at Nokia research Center and Nokia Networks, Helsinki. From 2004 to 2009 he was with Emirates Telecommunications Corporation, UAE. Also, from 2004 to 2013 he was adjunct Professor at the Department of Communications Engineering, TUT. His current research interests include mobile and broadband wireless communication systems, Mobile Edge Computing, Internet of Everything, and Machine Learning. In these areas, he has published over 200 journal and conference papers most of them in the peered reviewed IEEE publications, filed seven US patents, and wrote numerous confidential industrial research reports.  Dr. Hamila has been involved in several past and current industrial projects, Ooreedo, Qatar National Research Fund, Finnish Academy projects, EU research and education programs. He supervised a large number of under/graduate students and postdoctoral fellows. He organized many international workshops and conferences. He is a Senior Member of IEEE.

==> biographies/khan.tex <==
% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{biographies/khan.jpg}}]{Muhammad Asif Khan} (SM'20) received the B.Sc. degree in Telecommunication Engineering from University of Engineering and Technology Peshawar, Pakistan (2009) and M.Sc. in Telecommunication Engineering from University of Engineering and Technology Taxila, Pakistan (2013). He received the Ph.D. degree in Electrical Engineering from Qatar University in 2020. He was a Researcher Assistant at Qatar University (2014-2015) and at Qatar Mobility Innovation Center (2016-2017). He is currently working as a postdoctoral researcher at Qatar University. His current research interests include wireless communication, mobile edge computing, and distributed machine learning. He is a Senior Member of IEEE and a Member of IET. For more detailed information, please visit his homepage: \url{http://www.asifk.me}.
% \end{IEEEbiography}


%% Other journals using picinpar package
% \parpic{\includegraphics[width=1in,clip,keepaspectratio]{biographies/khan.jpg}}
% \noindent {\bf Muhammad Asif Khan} received the B.Sc. degree in Telecommunication Engineering from University of Engineering and Technology Peshawar, Pakistan (2009) and M.Sc. in Telecommunication Engineering from University of Engineering and Technology Taxila, Pakistan (2013). He received the Ph.D. degree in Electrical Engineering from Qatar University in 2020. He was a Researcher Assistant at Qatar University (2014-2015) and at Qatar Mobility Innovation Center (2016-2017). He is currently working as a postdoctoral researcher at Qatar University. His current research interests include wireless communication, mobile edge computing, and distributed machine learning. He is a Senior Member of IEEE and a Member of IET.
% % For more detailed information, please visit his homepage: \url{http://www.asifk.me}.

% \authorbiography[scale=0.3,overhang=0pt,wraplines=9,imagewidth=3cm,imagepos=]{biographies/khan.jpg}{Muhammad Asif Khan}
% {received the B.Sc. degree in Telecommunication Engineering from University of Engineering and Technology Peshawar, Pakistan (2009) and M.Sc. in Telecommunication Engineering from University of Engineering and Technology Taxila, Pakistan (2013). He received the Ph.D. degree in Electrical Engineering from Qatar University in 2020. He was a Researcher Assistant at Qatar University (2014-2015) and at Qatar Mobility Innovation Center (2016-2017). He is currently working as a postdoctoral researcher at Qatar University. His current research interests include wireless communication, mobile edge computing, and distributed machine learning. He is a Senior Member of IEEE and a Member of IET. For more detailed information, please visit his homepage: \url{http://www.asifk.me}}

% \begin{wrapfigure}{l}{23mm} \includegraphics[width=1in,height=2.4in,clip,keepaspectratio]{biographies/khan.jpg} \end{wrapfigure}
% \small

% \textbf{Muhammad Asif Khan} received a B.Sc. degree in Telecommunication Engineering from the University of Engineering and Technology Peshawar, Pakistan (2009) and an M.Sc. in Telecommunication Engineering from the University of Engineering and Technology Taxila, Pakistan (2013). He received a Ph.D. degree in Electrical Engineering from Qatar University in 2020. He was a Researcher Assistant at Qatar University (2014-2015) and at Qatar Mobility Innovation Center (2016-2017). He is currently working as a postdoctoral researcher at Qatar University. His current research interests include wireless communication, mobile edge computing, and distributed machine learning. He is a Senior Member of IEEE and a Member of IET. For more detailed information, please visit his homepage: \url{www.asifk.me}

\textbf{Muhammad Asif Khan} is an awarded post-doctoral research fellow at Qatar University. He received a Ph.D. degree in Electrical Engineering from Qatar University. His current research interests include visual crowd analysis, distributed machine learning, and edge intelligence. He is a Senior Member of IEEE and a Member of IET. For more detailed information, please visit his homepage: \url{www.asifk.me}


==> figures/fig1.tex <==



\begin{figure*}
\centering

\subcaptionbox{\scriptsize Crowd counting.}{
\includegraphics[width=4cm, height=2.5cm]{images/counting.jpg}}
\hspace{1em}
\subcaptionbox{\scriptsize Object detection.}{
\includegraphics[width=4cm, height=2.5cm]{images/obj_detection.jpg}}
\hspace{1em}
\subcaptionbox{\scriptsize Motion analysis.}{
\includegraphics[width=4cm, height=2.5cm]{images/motion.jpg}}
\\ \vspace{1em}


\subcaptionbox{\scriptsize Behavior analysis.}{
\includegraphics[width=4cm, height=2.5cm]{images/behavior.png}}
% \subcaptionbox{\scriptsize Activity recognition.}{
% \includegraphics[width=3cm, height=2cm]{images/activity.png}}
\hspace{1em}
\subcaptionbox{\scriptsize Anomaly detection.}{
\includegraphics[width=4cm, height=2.5cm]{images/anomaly.jpg}}
\hspace{1em}
% \subcaptionbox{\scriptsize Context analysis.}{
% \includegraphics[width=3cm, height=2cm]{images/context.jpg}}
% \hspace{1em}
\subcaptionbox{\scriptsize Crowd prediction.}{
\includegraphics[width=4cm, height=2.5cm]{images/context.jpg}}



\caption{Visual crowd analysis: Key areas of interest with examples.}
\label{fig1}
\end{figure*}

==> tables/tab-counting.tex <==



\begin{table*}[!h]
\centering
% \scriptsize
\caption{\rev{\scriptsize A summary of research efforts in crowd counting, categorized in distinct categories i.e., model architecture, loss functions, metrics, and training methods.}} \label{tab-counting}
\resizebox{\textwidth}{!}{  \colorbox{color1}{

\begin{tabular}{c p{12cm}} \toprule \\
Research Area &Summary of the SOTA  \\[0.5em] \midrule
& \\[0em]
Model Architectures
&Single-column \cite{CrowdCNN_CVPR2015}, multi-column \cite{MSCNN_ICIP2017}, Encoder-decoder \cite{TEDnet_CVPR2019}, pyramid, Vision transformers \cite{TransCrowd_2022} \\[3em]

Loss functions 
&Euclidean loss \cite{MCNN_CVPR2016}, Combination loss \cite{CrowdCNN_CVPR2015}, Curriculum Loss \cite{SGANet_IEEEITS2022}, Composite loss \cite{CompositionLoss_2018}, AP Loss \cite{ASNet_CVPR2020}, PRA Loss \cite{ASNet_CVPR2020}, SCL Loss \cite{TEDnet_CVPR2019}, OT \cite{DMCount_NeuroIPS2020}\\[4em]

Evaluation metrics
& MAE, MSE, GAME \cite{GAME_metric2015}, SSIM \cite{CSRNet_CVPR2018}, PSNR \cite{CSRNet_CVPR2018}, PAME \cite{}, PMSE \cite{}, MPAE \cite{} \\[2em]

Training methods
& Supervised/weakly-supervised \cite{Yang_ICCV2020, TransCrowd_2022, MATT_Elsevier_PR2020}, curriculum learning \cite{Khan2023LCDnet} \\[1.5em]
\bottomrule
\end{tabular}
}
}
\end{table*}

==> tables/tab-detection.tex <==





\begin{table}[!h]
\centering
% \scriptsize
\caption{\rev{\scriptsize A summary of object detection models.}} \label{tab-detection}
\resizebox{\columnwidth}{!}{  \colorbox{color1}{

\begin{tabular}{p{2.5cm} p{5cm}} \toprule \\
Model Category & Examples  \\[0.5em] \midrule
& \\[0em]


Anchor-based 
& FasterRCNN \cite{FasterRCNN_2015}, SSD \cite{SSD_2015}, YOLO \cite{} \\[3em]

Anchor-free 
& CornerNet \cite{CornerNet_2018}, CenterNet \cite{CenterNet_2019}, FCOS \cite{FCOS_2019}
\\[3em]

Transformer models
& Vision transformers (ViT) \cite{ViT_2022} \\[1em]
\bottomrule
\end{tabular}
}
}
\end{table}

==> tables/tab-summary.tex <==




\begin{table*}
\centering
\caption{\scriptsize Crowd analysis tasks and Open research problems.} \label{tab-summary}
\resizebox{\textwidth}{!}{ \colorbox{color1}{
% \scriptsize
\begin{tabular}{p{3cm} p{7cm} p{6cm}} \toprule 
&& \\[-0.5em]
\textbf{Crowd Analysis} & \textbf{Example Tasks}  & \textbf{Open Challenges} \\[1em] \midrule 

Crowd Counting
& Find the total headcount in a frame. \newline 
crowd localization in a large region. \newline
% & Multi-column CNNs, encoder-decoder models, pyramid networks  
& \rev{Handling severe occlusions, scale variations in highly dense crowd images, perspective distortion, multi-view counting.}
\\ [4em]

Object Detection 
& Detect and localize objects of interest. \newline 
Track objects in a video.
% & anchor-based (e.g., Faster-RCNN, YOLOv2), anchor-free (e.g., YOLO, FCOS, CornerNet, CenterNet)
& \rev{Viewpoint variations, Object deformation, severe occlusions, clutter, illumination, etc.}
\\ [3em]

Motion Analysis
& Observe crowd collectiveness. \newline
Is the crowd slow/fast-moving? \newline
Where is the crowd heading? at which speed? \newline
Find trajectories and motion patterns. \newline
% &optical flow, particle flow, spatiotemporal features.
& \rev{Complex semantic features, complex relationship between low-level pictorial features with high-level semantic features.}
\\ [4em]

Behavior/Activity Analysis
& Is the crowd calm or active? \newline
Are people protesting, dancing, fighting, etc?
% & Combination of methods (i.e., optical flow, LSTM, CNN etc.)
&\rev{Complex mapping of low-level features to activities, semantic relationship and mapping of detected activities to human behavior, standard activity definitions to semantic behavior.}\\ [5em]

Anomaly Detection
& Detect abandoned objects. \newline 
Detect any weapons or crimes? \newline
Detect intrusion.
% & k-means, SVM, GMM, CNNs, LSTMs, etc.
& \rev{Lacks of a unified definition of anomalies, lack of realistic datasets, huge size of video datasets \footnote{An extensive list of challenges can be found in \cite{Sharif2022DeepCA}}.}
\\ [3em]

Crowd prediction
& Detect if a crowd is expected in a region? \newline 
How crowd accumulates over time?
% & ARIMA, CNNs, LSTM, GNNs 
& \rev{Difficult to capture dual (spatial and temporal) dependencies, complex motion patterns.} \\ [1em]
\bottomrule
\end{tabular}
}
}
\end{table*}

==> tables/tab-surveys.tex <==







\begin{table*}[!h] \centering
\caption{\rev{\scriptsize Related studies on crowd visual analysis.}} \label{tab-surveys}
\resizebox{\textwidth}{!}{  \colorbox{color1}{

\begin{tabular}{p{4cm} p{3cm} p{10cm}} \toprule \\
Ref & Topic  & Brief Scope  \\[0.5em] \midrule
& \\[-0.5em]

\cite{Sindagi_2018} & Crowd counting &Methods, model architectures, datasets, future insights \\[0.5em]
\cite{Naveed_2020} & Crowd counting &Methods, model architectures, performance evaluation. \\[0.5em]
\cite{Gao_2020} & Crowd counting &Model architectures and categorization, datasets, evaluation metrics, challenges, and insights. \\[1.5em]
% \cite{Luo_2020} & Crowd counting &Summary \\[0.5em]
\cite{Gouiaa_2021} & Crowd counting &Methods, the taxonomy of CNN models, datasets, and applications. \\[1.5em]
\cite{Fan_2022} & Crowd counting &Methods, applications, and models. \\[0.5em]
\cite{khan2022revisiting} & Crowd counting &Datasets, model architecture, loss functions, evaluation metrics, insights \\[1.5em]

\cite{Hu2004ASO} &Motion analysis &Motion analysis, behavior analysis, moving object classification and identification. \\[1.5em]
\cite{Luca2020ASO} &Motion analysis &Flow prediction, next-location prediction, flow generation, and trajectory generation. \\[1.5em]

\cite{Kumar2021CrowdBM} &Behavior analysis &Methodologies for the organized crowd and non-organized crowd, datasets. \\[1.5em]

\cite{Modi2022ASO} & Anomaly detection &Methods for anomaly detection with merits and demerits. \\[0.5em]
\cite{Sharif2022DeepCA} &Anomaly detection & Methods, algorithms, datasets, and metrics with details analysis and comparisons.  \\[1.5em]

\cite{Li2015CrowdedSA} & Crowd analysis &Models, datasets, algorithms, and evaluation of crowd motion analysis, behavior recognition, and anomaly detection.  \\[1.5em]
\cite{HY2017CrowdBA} &Crowd analysis &Density estimation, motion detection and tracking, and behavior recognition. \\[1.5em]
\cite{Zhang2018PhysicsIM} &Crowd analysis &Physics-inspired methods for crowd video analysis. \\



\\[-0.5em]
\bottomrule
\end{tabular}
}
}
\end{table*}

==> tables/tab_detection2.tex <==





\begin{table}[!h]
\centering
% \scriptsize
\caption{\rev{\scriptsize A summary of object detection models.}} \label{tab-detection}
\resizebox{\columnwidth}{!}{  \colorbox{color1}{

\begin{tabular}{p{2.5cm} p{5cm}} \toprule \\
Model Category & Examples  \\[0.5em] \midrule
& \\[0em]


Anchor-based 
& FasterRCNN \cite{FasterRCNN_2015}, SSD \cite{SSD_2015}, YOLO \cite{} \\[3em]

Anchor-free 
& CornerNet \cite{CornerNet_2018}, CenterNet \cite{CenterNet_2019}, FCOS \cite{FCOS_2019}
\\[3em]

Transformer models
& Vision transformers (ViT) \cite{ViT_2022} \\[1em]
\bottomrule
\end{tabular}
}
}
\end{table}
